TMID: A Comprehensive Real-world Dataset for Trademark Infringement Detection in E-Commerce

Annually, e-commerce platforms incur substantial financial losses due to trademark infringements, making it crucial to identify and mitigate potential legal risks tied to merchant information registered to the platforms. However, the absence of high-quality datasets hampers research in this area. To address this gap, our study introduces TMID, a novel dataset to detect trademark infringement in merchant registrations. This is a real-world dataset sourced directly from Alipay, one of the world's largest e-commerce and digital payment platforms. As infringement detection is a legal reasoning task requiring an understanding of the contexts and legal rules, we offer a thorough collection of legal rules and merchant and trademark-related contextual information with annotations from legal experts. We ensure the data quality by performing an extensive statistical analysis. Furthermore, we conduct an empirical study on this dataset to highlight its value and the key challenges. Through this study, we aim to contribute valuable resources to advance research into legal compliance related to trademark infringement within the e-commerce sphere. The dataset is available at https://github.com/emnlpTMID/emnlpTMID.github.io .

==> p2_old_version.tex <==

%\subsection{Compliant Fund Advertising.}
% legal info
% Problem Formulation

%基金公司制作电子形式的广告，在电商平台上进行投放

% what is trademark, scope, question description
%A trademark is a type of intellectual property consisting of a recognizable sign, design, or expression that identifies products or services from a particular source and distinguishes them from others. Trademark IP protection is based on the Intellectual Property Trademark Protection Law. From a legal perspective, the following definitions of relevant terms apply to trademark infringement protection:
%Similar trademark: Refers to the accused trademark compared with the plaintiff's registered trademark, with similar shape, pronunciation, meaning, composition of graphics and colors, or the overall structure of the combination of its elements. The 3D shape, color combination is also similar, which easily leads to confusion among the relevant public about the source of the goods or to believe that there is a specific association with the plaintiff's registered trademark.
%Similar goods: Refers to goods that have the same function, use, production department, sales channel, consumer objects, or are generally considered by the public to have specific associations, which easily leads to confusion.
%Similar services: Refers to services that have the same purpose, content, method, object, or are generally considered by the public to have specific associations, which easily leads to confusion.

%On e-commerce platforms, the typical problem is that a merchant might risk infringing the trade mark IP rights of protected trademark owners, which can be individuals, business organizations, or any legal entity, intentionally or unintentionally. However, IP infringement can happen at arbitrary places when the merchant is selling its goods. In contrast to the previous work, which only considers trademark infringement detection as a logo similarity measure, the scope of our scenarios is much larger. Therefore, we need comprehensive information on censored merchants to assess their risk of IP infringement. 
% https://www.gov.uk/guidance/unacceptable-trade-marks

A trademark is a valuable form of intellectual property encompassing a distinctive sign, design, or expression used to identify and differentiate products or services from one source to another\footnote{https://www.gov.uk/guidance/unacceptable-trade-marks}. Various laws across different countries carefully define the infringement of trademark IP rights. As our data source is from a Chinese e-commerce platform, the scope of the infringement is defined by the respective law of the People's Republic of China, as outlined in Appendix~\ref{app:trade_law}.

E-commerce platforms face significant financial risks when merchants on their platforms potentially infringe on the intellectual property rights of trademark owners, who can be individuals, businesses, or legal entities. To address this issue, our team of legal experts abide by the trademark IP protection law, which outlines the following summary of trademark infringement by merchants on an e-commerce platform:

\begin{table}
\centering
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{ccc}
\hline
     type1  & type2 & type3    \\
\hline
2 & 14 & 123      \\
\hline
\end{tabular}}
\caption{
Statistics of reasoning traces.
}
    \vspace*{-6mm}
\label{background data statistics}
\end{table}

\begin{itemize}[leftmargin=*]
    \item Use of similar trademarks: This refers to merchants using trademarks that bear resemblance to other registered trademarks in terms of shape, pronunciation, meaning, the composition of graphics and colours, or the overall combination of elements. %It includes cases where the accused trademark's 3D shape or colour combination is also similar, leading to potential confusion among the relevant public regarding the origin of the goods or implying a specific association with the registered trademark.
    \item Sale of similar goods: This pertains to scenarios where merchants, even when using different trademarks, sell goods that serve the same purpose, have the same use, are produced by the same manufacturer, are sold through the same distribution channels, and target similar consumers. The similarity among these goods can easily lead to confusion among the public.
    \item Provision of similar services: This refers to situations where merchants, despite employing different trademarks, provide services with the same objective, content, method, or targeting the same audience.
    %The public can also perceive similar services as having specific associations, which may confuse them.
\end{itemize}

%在数据集中，有192条的数据被标注了推理原因，192条数据中有139条数据侵犯了知名品牌的商标注册权，对推理原因进行了相应的类别统计，数据显示在Table1里，其中type1代表use of similar trademarks only, type2代表use of similar trademarks and sale of similar goods, type3代表use of similar trademarks and provision of similar services.
In the dataset, 192 pieces of data have been annotated with reasoning traces. Among the 192 pieces of data, 139 have infringed on the trademark registration rights of well-known brands. The corresponding category statistics were conducted on the inference reasons, and the data is shown in Table\ref{background data statistics}. Among them, type 1 represents the use of similar trademarks only, type 2 represents the use of similar trademarks and sale of similar goods, and type 3 represents the use of similar trademarks and provision of similar services.

 These infringement cases on e-commerce platforms are difficult to detect as they can occur at any phase of the merchant's sales process, in various forms and often in unforeseen manners. Unlike previous approaches that naively consider logo similarity for trademark infringement detection~\cite{trappey2020intelligent}, our task is more complex, focusing on a broader range of scenarios. Therefore, we require comprehensive information when censoring merchants to evaluate their risk of trademark infringement.

In our context, trademark infringement detection involves determining whether a censored merchant on the e-commerce platform risks infringing upon the trademark IP laws regarding a protected trademark registered by the trademark owner. We can formalize this task by defining a function:
\begin{equation}
\pi_{\theta} : \mathcal{X}{s} \times \mathcal{T}{p} \times \mathcal{R} \rightarrow \{0,1\}
\end{equation}
Here, $x_s \in \mathcal{X}{s}$ represents the collected information of the merchants to be censored, while $t_p \in \mathcal{T}{p}$ corresponds to the information of the protected trademarks. $R$ denotes the local law governing trademark IP protection. Specifically, the information of censored merchants consists of their registration details $x^{r}_s$ on the platform and externally acquired information $x^{p}_s$, represented as $x_s = \{x^{r}_s, x^{p}_s\}$. On the other hand, the data of protected trademarks include their unique trademark identifiers, denoted as $t_{p}^i$, and auxiliary information denoted as $t_{p}^{a}$. More detailed explanations regarding each type of information will be provided in Section~\ref{sec:trademark}.

%Similar trademark: This refers to a trademark that bears resemblance to the plaintiff's registered trademark in terms of shape, pronunciation, meaning, composition of graphics and colors, or overall combination of its elements. It includes cases where the accused trademark's 3D shape or color combination is also similar, leading to potential confusion among the relevant public regarding the origin of the goods or implying a specific association with the plaintiff's registered trademark.

%Similar goods: This refers to goods that serve the same purpose, have the same use, are produced by the same department, sold through the same channels, target similar consumers, or are generally perceived by the public to have specific associations. The similarity among these goods can easily lead to confusion.

%Similar services: This refers to services that have the same objective, content, method, or target the same audience. Similar services can also be perceived by the public as having specific associations, which may cause confusion.



%A trademark may be located on a package, a label, a voucher, or on the product itself. Trademarks used to identify services are sometimes called service marks.

%与过去的学术论文定义相比，本文中定义的trademark的范围有所不同。比如在文章中(https://www.mdpi.com/2076-3417/12/3/1752)将trademark定义为一个recognizable sign，提供了一种基于CNN的检查待注册商标的图标与历史已注册图标间的图像相似度的方法。本文中定义的商标不仅局限于用于识别某企业的图形形式的显著标志，而是包括了图形和文字形式的用于识别某企业的显著标志。
%In contrast to prior academic papers, the scope of the trademark in this paper exhibits slight variations. For instance, as explicated in the article (https://www.mdpi.com/2076-3417/12/3/1752), the trademark is conceptualized as a recognizable sign, with a CNN-based method provided to assess the resemblance between the icon image of a pending trademark registration and that of a historically registered trademark. Notably, the definition of the trademark in this study extends beyond prominent graphic symbols used to identify a company, encompassing symbols in both graphic and textual forms.

%Trademark IP Protection 基于知识产权-商标权保护法。从法律角度出发，商标权侵权保护中相关的名词定义如下：
%近似商标：是指被控侵权的商标与原告的注册商标相比较，其文字的字形、读音、含义或者图形的构图及颜色，或者其各要素组合后的整体结构相似，或者其立体形状、颜色组合近似，易使相关公众对商品的来源产生误认或者认为其来源与原告注册商标的商品有特定的联系。
%类似商品：是指在功能、用途、生产部门、销售渠道、消费对象等方面相同，或者相关公众一般认为其存在特定联系，容易造成混淆的商品。
%类似服务：是指在服务的目的、内容、方式、对象等方面相同，或者相关公众一般认为存在特定联系，容易造成混淆的服务。
%Trademark IP protection is based on the Intellectual Property Trademark Protection Law. From a legal perspective, the following definitions of relevant terms apply to trademark infringement protection:
%Similar trademark: Refers to the accused trademark compared with the plaintiff's registered trademark, with similar shape, pronunciation, meaning, composition of graphics and colors, or the overall structure of the combination of its elements. The 3D shape, color combination is also similar, which easily leads to confusion among the relevant public about the source of the goods or to believe that there is a specific association with the plaintiff's registered trademark.
%Similar goods: Refers to goods that have the same function, use, production department, sales channel, consumer objects, or are generally considered by the public to have specific associations, which easily leads to confusion.
%Similar services: Refers to services that have the same purpose, content, method, object, or are generally considered by the public to have specific associations, which easily leads to confusion.

%\section{Compliant Fund Advertising}

==> prior_intro.tex <==
As Internet applications and e-commerce develop rapidly, in order to provide electronic services, more and more merchants are starting to enter electronic platforms such as Alipay, WeChat, etc., in the form of Mini-Apps. Taking Alipay as an example, by the end of 2022, more than 200 thousand merchants have registered in the form of Mini-Apps on the electronic platform. ...

After registering on electronic platforms, merchants often advertise their business categories or provided services in order to increase the click rate of their registered Mini-Apps. In some cases, they may use the names of well-known brands in their certification information without prior authorization, riding the wave of the well-known brand's popularity to illegally gain profits. This kind of behavior is a violation of the well-known brand's intellectual property rights, causing detriment to its legitimate interests. To prevent this occurrence, we propose to employ deep learning based methods to solve the intellectual property infringement checking problem. Considering the peculiarities of the Mini-Apps, it is essential to take into account all available inputs and synthetically consider all the information to evaluate if any illegal activity presents. ...

Fig.1 Example of the Mini-App
Fig.2 Procedure of the intellectual property infringement review

Infringement review of intellectual property is a typical classification problem; however, it faces three main challenges. 
(1) It is difficult to comprehensively consider all the available information from what the merchant has submitted to the electronic platform in order to accurately judge whether infringement exists, and to accurately determine which part of the information is infringing due to the Mini-Apps' particularity. 
(2) As shown in Fig.2, an authorization library is used to filter out official certified merchants; however, this manual process is low efficiency and has no real-time guarantee, leading to incompleteness of data almost all the time. Thus, in order to infer whether there is an industrial or business relationship between the registered merchant and the suspected infringing brand, advanced algorithms must be employed. 
(3) Additionally, in some infringing cases, the registered merchant is an offline store which provides sale service for a well-known brand; this kind of relationship is not maintained in our database. To identify this situation, advanced algorithms must be used to find out such a relationship.

So we propose to ...

The contribution can be summarized as follows:
(1) We define the infringement review of intellectual property task on Mini-Apps, which aims to ... 
(2) A huge deep learning based supply chain map ... 
(3) A Dataset ... 
(4) We propose to apply the supply chain map on the infringement review of intellectual property task on Mini-Apps ...

\begin{itemize}
    \item The first real-world comprehensive trademark application dataset for legal risk detection, including logos, textual descriptions, signature, comprehensive background knowledge, such as merchant information, statutes, judgements.
    \item Manually annotated reasoning traces, understandable by both legal professionals and computer scientists without special training.
    \item The first real-world dataset for detecting legal risks in investment fund advertisements.
    \item Conduct the first empirical study on both datasets, with the following findings.
\end{itemize}
